Sampling cluster point processes: a review

The theme of this article is the sampling of cluster and iterated cluster point processes. It is partially a review, mainly of the Brix-Kendall exact sampling method for cluster point processes and its adaptation by M{\o}ller and Rasmussen to Hawkes branching point processes on the real line with light-tail fertility rate are reviewed. The main novel aspect of this review is the extension to non-Poissonian germ point processes. For this, a slight adaptation is needed. A formal proof via Laplace transforms of the validity of the method in terms of general clusters that are not necessarily point processes fits this purpose and allows to include the exact sampling of Boolean models.

==> brem_input.tex <==

%%%%%%%%%%%begin Pam's modifications to book.sty
\typeout{ }
\typeout{book.sty : Modified 1/16/96 by}
\typeout{PWILLIAMS@ECS.UMASS.EDU}
\typeout{ }
\setlength {\textwidth}{6.5truein}
\setlength {\oddsidemargin}{0truein}
\setlength {\evensidemargin}{0truein}
\def\ul{\underline}
\def\hb{\hbox}
\def\vs{\vskip}
\def\sk{\vskip.1in}   
\def\cov{\;\hbox{cov}\;}
\def\Var{\;\hbox{Var}\;}
\def\ub{\underline}
\def\square{\vrule height 0.5em width 0.4em depth-0.1em}
%%%selected caligraphy characters
\def\O{{\cal O}}
\def\D{{\cal D}}
\def\A{{\cal A}}
\def\Q{{\cal Q}}
\def\S{{\cal S}}
\def\T{{\cal T}}
\def\U{{\cal U}}
\def\W{{\cal V}}
\def\Y{{\cal Y}}
\def\I{{\cal I}}
\def\X{{\cal X}}
\def\K{{\cal K}}
\def\N{{\cal N}}
\def\C{{\cal C}}
\def\E{{\cal E}}
\def\B{{\cal B}}
\def\X{{\cal X}}
\def\L{{\cal L}}
\def\Z{{\cal Z}}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal H}}
\def\V{{\cal V}}
\def\R{{\cal R}}
\def\M{{\cal M}}
\def\P{{\cal P}}
\def\b1{{\bf 1}}
\def\bZ{{\bf Z}}
\def\bF{{\bf F}}
\def\bG{{\bf G}}
\def\bQ{{\bf Q}}
\def\bR{{\bf R}}
\def\bP{{\bf P}}
\def\bI{{\bf I}}
\def\bN{{\bf N}}
\def\bO{{\bf O}}


%%%%%selected characters with bars over them.
\def\bC{\bar C}\def\bM{\overline{M}}\def\bD{\bar D}\def\bB{\bar
B}\def\bA{\bar A} 
\def\bbR{\bar\R}
\def\ua{\underline{a}}

%%%%%%constructed characters
\def\deleq{\stackrel{\Delta}{=}}
\def\defeq{\stackrel{\rm def}{=}}
\def\tow{\stackrel{\rm w}{\to}}
\def\toL{\stackrel{\cal L}{\to}}

%%%%%%%short cuts
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\ban}{\begin{eqnarray}}
\newcommand{\ean}{\end{eqnarray}}

\def\beq#1\eeq{\begin{equation}#1\end{equation}}

%\def\pmatrix#1{\begin{pmatrix} #1 \end{pmatrix}}
%\def\bmatrix#1{\begin{bmatrix} #1 \end{bmatrix}}
%\def\matrix#1{\begin{matrix} #1 \end{matrix}}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}

\newcommand{\bc}{\left\{\begin{array}{cl}}
\newcommand{\ec}{\end{array}\right.}
\newcommand{\be}{\begin{displaymath}}
\newcommand{\ee}{\end{displaymath}}
\def\ben{\begin{eqnarray*}}
\def\een{\end{eqnarray*}}
\def\var{\;\hbox{Var}\;}
\def\rmsinc{\;\hbox{since}\;}
\def\rman{\;\hbox{and}\;}
\def\rmor{\;\hbox{or}\;}
\def\rmfor{\;\hbox{for}\;}
\def\rif{\;\hbox{if}\;}
\def\mod{\;\hbox{mod}\;}
\def\card{\;\hbox{card}\;}
\def\where{\;\hbox{where}\;}
\def\Cup{\bigcup}
\def\Cap{\bigcap}
\def\case{\left\{\begin{array}{ll}}
\def\ecase{\end{array}\right.}
%*****rajoute********
\def\ie{\textit{i.e.,}\;}
%*******************
%%%%%%%%%more hats and bars and character format shortcuts
\def\tY{\tilde Y}
\def\tZ{\tilde Z}
\def\tS{\tilde S}
\def\hbP{\bar\bP}
\def\bbR{\bar\R}
\def\hX{\hat X}
\def\hZ{\hat Z}
\def\hY{\hat Y}
\def\C{\cal C}
\def\inf{\;\hbox{inf}\;}
\def\for{\;\hbox{for}\;}
\def\resp{\;\hbox{resp}\;}
\def\diag{\;\hbox{diag}\;}
\def\Adj{\;\hbox{Adj}\;}
\def\foral{\;\hbox{for all}\;}
\def\signline{\vrule height1pt width 1in depth-.05pt}
\def\tA{\tilde A}
\def\tD{\tilde D}

%%%%%%DEFINITION to get ONE, TWO, etc for chapters
\catcode`\@=11
\def\Typeo#1{\ifcase\csname c@#1\endcsname
Zero\or One\or Two\or Three\or Four\or Five\or Six\or Seven\or Eight\or Nine
\or Ten\or Eleven\fi}

%%%%%reformatting type of counters for sections, etc.
\def\thepart {\Roman{part}}
\def\thechapter {\arabic{chapter}}
\def\thesection {\arabic{section}}
\def\thesubsection {\thesection.\arabic{subsection}}
%\def\thesubsection {}%{\thesection.\arabic{subsection}}
\def\thesubsubsection {}%{\thesubsection.\arabic{subsubsection}}
\def\theparagraph {\thesubsubsection.\arabic{paragraph}}
\def\thesubparagraph {\theparagraph.\arabic{subparagraph}}
\def\@chapapp{Chapter}
\@addtoreset{equation}{section} 
\def\theequation{\thesection.\arabic{equation}}

\def\thefigure{\@arabic\thesection.\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\bf figure \thefigure}
\def\figure{\@float{figure}}
\let\endfigure\end@float
\@namedef{figure*}{\@dblfloat{figure}}
\@namedef{endfigure*}{\end@dblfloat}
\@addtoreset{figure}{section}
\def\theproblems{\@arabic\thesection.\@arabic\c@problems}

%%%definitions for theorem, definition, example and proof.
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{exercise}{Exercise}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{problems}{Problems}[section]
\def\enex{{\hfill$\Diamond$}}
\def\enrem{{\hfill$\Diamond$\sk}}
\def\enpro{{\hfill$\Box$\sk}}


\def\noi{\noindent}

\def\ul{\underbar}
\def\comment{\noi\ul{\bf Comment.}\ \ }
\def\hint{\noi\ul{\bf Hint.}\ \ }
\def\proof{\noi{\bf Proof.}\ \ }
%\def\proof{\noi\ul{\bf Proof.}\ \ }
\def\solution{\noi\ul{\bf Solution.}\ \ }
%\def\proofs{\noi\ul{\bf Proofs.}\ \ }

\def\notation{\noi\ul{\bf Notation.}\ \ }

%%%%%%%theorem environment  NOT BEING USED
%\def\theorem#1{\begin{tabular}{|p{6in}|}\hline\\
%\vspace{-24pt}\begin{theorem} %
%{#1}\end{theorem}\\
%\hline\end{tabular}}

% Redefine theorem environment macros to put \theoremcounterend
% (default ".") after the "theorem" head.

\def\@begintheorem#1#2{\rm \trivlist
   \item[\hskip \labelsep{\bf #1\ #2\thmcounterend}]}
\def\@opargbegintheorem#1#2#3{\rm \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3)\thmcounterend}]}
\def\thmcounterend{.}

%definitions rajoutees par Philippe
\def\pth#1{\left(#1\right)}
\def\acc#1{\left\{#1\right\}}
\def\cro#1{\left[#1\right]}
\def\bars#1{\left|#1\right|}
\def\norm#1{\left\|#1\right\|}
\def\egdef{\stackrel{\Delta}{=}}

%defintion de l'environnement proof 
%    \newenvironment{proof} 
%    {%preambule
%     %definition du titre de proof
     
%      \noindent \footnotesize\textbf{Proof}
%      \slshape %font du texte de proof 
%    } %fin du preambule 
%    {%postambule
     %defintion du cube de fin de proof
%     \nobreak\hfill$\Box$ 
%    }%fin du postambule

%redefintion de l'environnement example 
 %   \renewenvironment{example}
  %  {%preambule
     %increment du compteur
  %   \refstepcounter{example}
     %definition du titre de l'example
   %  {
   %   \noindent \textbf{Example~\theexample}{\color{backgroundgray} %\mbox{\hrulefill}\par\nobreak }}
      %N.B. \theexample montre la valeur du compteur example
    %  \normalfont %font du texte de l'example 
    %} %fin du preambule 
    %{%postambule
     %defintion de la ligne de fin example
    % \par\nobreak{\color{backgroundgray} \noindent\rule{\linewidth}{1mm}} 
    %}%fin du postambule  




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "innit"
%%% End: 

